Constraints Satisfiability Driven Reinforcement Learning for Autonomous Cyber Defense

With the increasing system complexity and attack sophistication, the necessity of autonomous cyber defense becomes vivid for cyber and cyber-physical systems (CPSs). Many existing frameworks in the current state-of-the-art either rely on static models with unrealistic assumptions, or fail to satisfy the system safety and security requirements. In this paper, we present a new hybrid autonomous agent architecture that aims to optimize and verify defense policies of reinforcement learning (RL) by incorporating constraints verification (using satisfiability modulo theory (SMT)) into the agent's decision loop. The incorporation of SMT does not only ensure the satisfiability of safety and security requirements, but also provides constant feedback to steer the RL decision-making toward safe and effective actions. This approach is critically needed for CPSs that exhibit high risk due to safety or security violations. Our evaluation of the presented approach in a simulated CPS environment shows that the agent learns the optimal policy fast and defeats diversified attack strategies in 99\% cases.

==> use_case.tex <==
\section{Case Study}
\begin{figure}
    \centering
    \includegraphics[height=4.3cm,width=11cm]{figs/aica_ddos.pdf}
	\caption{Use Case Study: Deploying Autonomous Agents to defend Volumetric DDoS Attack. Agent $m_1$ is responsible to protect sub-domain 1 including link $L_1$, and $m_2$ is responsible to protect sub-domain 2 including link $L_2$. $H_{i}$ represents end host or server or service, $S_i$ represents switch or router, and $L_1$ or $L_{i,j}$ represents links.} 
	%A strategy is verified if it satisfies all constrains during that phase (pre/post).}
	\label{fig:use_case}
\end{figure}
To show the benefit and feasibility of our framework, we consider \textit{protecting an enterprise network from volumetric DDoS attack} as use case study. Fig. \ref{fig:use_case} illustrates the network, where switch $S_1$ connects three end-devices ($H_1$-$H_3$) and switch $S_2$ connects two end-devices ($H_4$-$H_5$) with the internet through a router $r_1$. There are two sub-domains: (1) sub-domain 1 with $S_1$ that is connected with $r_1$ through link $L_1$, and (2) sub-domain 2 with $S_2$ that is connected with $r_2$ through link $L_2$. All links $L_1$, $L_2$, and $L_{i,j}$ (connecting two nodes $i$ and $j$) have specific resource utilization, and any traffic over the utilization will be dropped. 

As shown in Fig. \ref{fig:use_case}, benign and attack sources can send traffic towards $H_1-H_5$, and any excessive traffic towards an end-device $H_i$ congests its relevant $L_i$ that induces traffic drop of all devices of that sub-domain. To clarify, huge traffic towards $H_1$ drops traffic of $H_2$ and $H_3$ alongside $H_1$ due to congesting link $L_1$. Therefore, attackers send traffic from distributed sources to launch attack against the enterprise network, and the enterprise hosts an Intrusion Detection System (IDS) before $r_1$ to distinguish between attack and benign flows. IDS quantifies the maliciousness of traffic based on its deviation from the normal traffic and provides as risk score $q\in [0,1]$. Generally, the defender drop a traffic as attack traffic if its IDS risk score $q$ is above than the threshold $\gamma$.

The most critical challenge in dealing with IDS lies in determining the optimal threshold; otherwise, false positive rate $f_p$ (i.e., identifying benign traffic as attack traffic) becomes high if $\gamma$ is less than optimal, and false negative rate $f_n$ (i.e., identifying attack traffic as benign traffic) becomes high if $\gamma$ is higher than the optimal. Moreover, optimal $\gamma$ differs for end-devices and traffic types (e.g., TCP, UDP). Therefore, the defender must determine optimal threshold $\gamma_i^k$ for an end-device $H_i$ and traffic type $k$, based on the current traffic condition, normal traffic behavior of the host, and others. 

\section{Problem Formulation}
\label{sec:problem_forms}

